Synthesizing Document Database Queries using Collection Abstractions

Document databases are increasingly popular in various applications, but their queries are challenging to write due to the flexible and complex data model underlying document databases. This paper presents a synthesis technique that aims to generate document database queries from input-output examples automatically. A new domain-specific language is designed to express a representative set of document database queries in an algebraic style. Furthermore, the synthesis technique leverages a novel abstraction of collections for deduction to efficiently prune the search space and quickly generate the target query. An evaluation of 110 benchmarks from various sources shows that the proposed technique can synthesize 108 benchmarks successfully. On average, the synthesizer can generate document database queries from a small number of input-output examples within tens of seconds.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

ACMCPSAMPLES= \
	samples/sample-acmcp-Discussion.pdf \
	samples/sample-acmcp-Invited.pdf \
	samples/sample-acmcp-Position.pdf \
	samples/sample-acmcp-Research.pdf \
	samples/sample-acmcp-Review.pdf \

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: ${ACMCPSAMPLES} acmart.cls
	zip $@ $+

samples/sample-acmcp.tex: samples/samples.ins samples/samples.dtx
	cd samples; pdflatex samples.ins; cd ..


samples/sample-acmcp-%.tex: samples/sample-acmcp.tex samples/acm-jdslogo.png
	sed 's/acmArticleType{Review}/acmArticleType{$*}/' $< > $@

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> figures/algo-abs-match.tex <==
\begin{figure}[!t]
\begin{algorithm}[H]
\caption{Match}
\begin{algorithmic}[1]
\Procedure{\textsc{Match}}{$\type, \augType$}
\vspace{2pt}
\Statex \textbf{Input:} A document type $\type$ and an augment type $\augType$
\Statex \textbf{Output:} $\top$ if $\type \matches \augType$ or $\bot$ otherwise
\vspace{2pt}

\State $\type_k \gets \cmdToDocType(\augType)$

\If{$\neg \type_k \subseteq \type$}
    \Return $\bot$
\Else
    \State $\type \gets \type - \type_k$
    \State $\augType \gets \augType - \type_k$
\EndIf
\State $L^1 \gets \set{\texttt{?}_i^m | \texttt{?}_i^m \in \augType \land m = 1}$
\For{$\text{each}~ \texttt{?}_i^m \in L^1$}
    \If{$\neg \exists a. a \!\in\! \type \land \textsl{InTopLevel}(a) \land (\textsl{Type}(a) \!=\! \textsl{Type}(\texttt{?}_i^m) \lor \textsl{Type}(\texttt{?}_i^m) = \cmdAny)$}
        ~\Return $\bot$
    \Else
        \State $\type \gets \type - \set{a: \textsl{Type}(a)}$
        \State $\augType \gets \augType - \set{\texttt{?}_i^m: \textsl{Type}(\texttt{?}_i^m)}$
    \EndIf
\EndFor
\State $L_T \gets [\textsl{Type}(\texttt{?}_i^m)| \texttt{?}_i^m \in \augType \land m = +]$
\State \Return \textsc{MatchMulti}$(\type, L_T)$

\EndProcedure


\Procedure{\textsc{MatchMulti}}{$\type, L_T$}
\If {$|L_T| = 0$}
    \Return \textsl{ite}$(\type = \set{}, \top, \bot)$
\EndIf
\If {$\type = \set{}$}
    \Return \textsl{ite}$(|L_T| = 0, \top, \bot)$
\EndIf
\If {$L_T[0] = \cmdAny$}
    \For {$j \gets 1 ~\text{to}~ \textsl{CountTopAttrs}(\type)$}
        \State $\type' \gets \textsl{DelTopAttrs}(\type, j)$
        \If {$\textsc{MatchMulti}(\type', L_T[1:])$}
            \Return $\top$
        \EndIf
    \EndFor
            
\Else 
    \For {$j \gets 1 ~\text{to}~ \textsl{CountTopAttrsWithType}(\type, L_T[0])$}
        \State $\type' \gets \textsl{DelTopAttrsWithType}(\type, L_T[0], j)$
        \If {$\textsc{MatchMulti}(\type', L_T[1:])$}
            \Return $\top$
        \EndIf
    \EndFor
\EndIf
\State \Return $\bot$

\EndProcedure

\end{algorithmic}
\end{algorithm}
\label{algo:abs-match}
\end{figure}


==> stale/fig-concrete-semantics-aux.tex <==
\begin{figure*}[!t]
% \framebox[\textwidth]{$\denot{\textsl{AttrFn}} ::= \doc \rightarrow \doc$}
\[
\begin{array}{rcl}
\cmdAddAttrs(\doc, \vec{h}, \vec{v}) &=& \cmdFoldl(\lambda \doc. \lambda (h, v). \cmdPut(\doc, h, v), \doc, \cmdZip(\vec{h}, \vec{v}))\\
\cmdExtractAttrs(\doc, \vec{h}) &=& \cmdFoldl(\lambda \doc. \lambda h. \cmdPut(\doc, h, \denot{h}_\doc), \set{}, \vec{h})\\
\cmdPut(\doc, h, v) &=& \cmdMergeWith(\doc, \cmdConstruct(h, v))\\
\end{array}
\]

% \framebox[\textwidth]{$\denot{\cmdConstruct} ::= h \rightarrow v \rightarrow v$}
\[
\begin{array}{rcl}
\cmdConstruct([], v) &=& v\\
\cmdConstruct((a: as), v) &=& \set{a: \cmdConstruct(as, v)}\\
\end{array}
\]

% \framebox[\textwidth]{$\denot{\cmdMergeWith} ::= \doc \rightarrow \doc \rightarrow \doc$}
\[
\begin{array}{rcl}
\cmdMergeWith(x, y) \\
    & | & \cmdIsDoc(x) \land \cmdIsDoc(y) = \set{a_{x1}: v_{x1}, \ldots, a_{xm}: v_{xm}, a_{y1}: v_{y1}, \ldots, a_{yn}: v_{yn}, \\
    & & a_p: \cmdMergeWith(v_{xp}, v_{yp}), \ldots, a_q: \cmdMergeWith(v_{xq}, v_{yq})} \\
    & & \qquad \text{where } x = \set{a_{x1}: v_{x1}, \ldots, a_{xm}: v_{xm}, a_p: v_{xp}, \ldots, a_q: v_{xq}} \text{ and } \\
    & & \qquad \qquad y = \set{a_{y1}: v_{y1}, \ldots, a_{yn}: v_{yn}, a_p: v_{yp}, \ldots, a_q: v_{yq}} \\
    & | & \text{otherwise} = y\\
\end{array}
\]

% \framebox[\textwidth]{$\denot{\cmdFlattenArr} ::= \doc \rightarrow \vec{\doc}$}
\[
\begin{array}{rcl}
\cmdFlattenArr(\doc, h) &=& \cmdMap(\lambda x. \cmdMergeWith(\doc, \cmdConstruct(h, x)), \denot{h}_\doc)\\
\end{array}
\]


\caption{Auxiliary Functions. }
\label{fig:concrete-semantics-aux}
\end{figure*}

